Characterizing and Predicting Email Deferral Behavior

Email triage involves going through unhandled emails and deciding what to do with them. This familiar process can become increasingly challenging as the number of unhandled email grows. During a triage session, users commonly defer handling emails that they cannot immediately deal with to later. These deferred emails, are often related to tasks that are postponed until the user has more time or the right information to deal with them. In this paper, through qualitative interviews and a large-scale log analysis, we study when and what enterprise email users tend to defer. We found that users are more likely to defer emails when handling them involves replying, reading carefully, or clicking on links and attachments. We also learned that the decision to defer emails depends on many factors such as user's workload and the importance of the sender. Our qualitative results suggested that deferring is very common, and our quantitative log analysis confirms that 12% of triage sessions and 16% of daily active users had at least one deferred email on weekdays. We also discuss several deferral strategies such as marking emails as unread and flagging that are reported by our interviewees, and illustrate how such patterns can be also observed in user logs. Inspired by the characteristics of deferred emails and contextual factors involved in deciding if an email should be deferred, we train a classifier for predicting whether a recently triaged email is actually deferred. Our experimental results suggests that deferral can be classified with modest effectiveness. Overall, our work provides novel insights about how users handle their emails and how deferral can be modeled.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

==> old.tex <==
\section{Old content moved}
\ms{Only made minor edits after here}
We are not aware of any past work that investigated the deferral behaviour using large scale log analysis. One main challenge with studying deferral through the logs of user-email interaction is to identify whether or not an email is deferred by the user. 
Deferral is best characterized by recognizing the intent of the user at the time of first email visit. However, as is common shortcoming of retrospective analysis, we can take advantage of users interactions with their messages as a proxy to their deferral intent. Following this approach, there are two ways we can define deferral:
\begin{enumerate}
	\item Explicit Deferral, where Revisit behaviour is a subset of Deferral;
	\item Implicit Deferral, where Deferral is a subset of Revisit behaviour;
\end{enumerate}

In the first case the Explicit Deferral defines the Revisit behaviour. In this definition Revisit is a subset of Deferral. That is, among all those emails that are explicitly deferred by the users (e.g. by marking as Unread or Flagging it), a subset of them will be revisited at a later time and a "strong action" such as Reply|ReplyAll|Forward.
However, an alternative way to look at Deferral / Revisit behaviour is to focus on Revisit itself independent from an observation of an explicit deferral case. This new point of view helps identify both explicit and implicit deferral.

To elaborate, during Triage as the user comes across an email and the email is read, we are not sure whether the user intended to defer his action on that email or not. But once we observe a revisit activity that includes a "strong action" like Reply|ReplyAll|Forward we can also infer that email was originally deferred.

\subsection{Proxey for Deferral}
TODO: Use the Qualitative data collected through interviews and the survey to show Response actions are a big part of Deferral scenarios. And it's also a clear scenario to analyze in the logs. So that's what we are using in our analysis to characterize deferral.
\subsection{Defining Revisit}
Closely coupled with the deferral of emails is how users revisit these deferred messages.  
According to Siu et al (2006) users revisit emails in two main ways:  
\begin{itemize}
	\item It occurs when users finish an activity and are waiting to move to their next task; 
	\item towards the end of the day when the pace of incoming mail is likely low and the user's time is likely free. 
\end{itemize}
Besides, the revisit activity (and hence the defer activity) is often task or issue oriented. 
	
We are interested to characterize this revisiting behavior associated with deferral as well. More specifically, we'd like to look at actions a user has taken immediately before he revisited a deferred email to take an action such as Reply. These actions can be available through the Email logs or the Web search logs (or possibly logs of other resources e.g. calendar, Windows, etc).

The revisit activity is distinct from the retrieve activity that Venolia et al. [20] described because revisit deals with deferred emails that may contain tasks, whereas the retrieve activity refers to archived emails that have been stored and already handled.  The revisit activity is also closely tied with handling email flow, whereas the retrieve activity is a form of information retrieval.     

\section{Research Questions and Prediction Tasks}
 \ms{repetitive; listed in intro}
	\textbf{[RQ1]:} What are the Characteristics of Deferred Email?\\
		a) Distributions of actions\\
		b) Distributions of time (between read and revisit)\\
	\textbf{[RQ2]}: What are the factors that lead to an email being deferred?\\ 
		a) Characteristics of the user's mailbox? (large mailbox, very structured mailbox, ...)\\
		b) Characteristics of the emails? (metadata + type of email)\\
		c) Characteristics of the users? (e.g. Filer vs Piler)\\
	\textbf{[RQ3]:} What are the reasons and rationales for deferring an email?\\ 
		a) Qualitative Study\\
	\textbf{[PT1]:} Given a delivered email, can we predict if it's going to be deferred?\\
	\textbf{[PT2]:} Given a Deferred Email, can we predict how soon the user will revisit to handle that email?\\ 

\section{Qualitative Analysis}
Our motivation with collecting some qualitative data using a series of interviews and survey is to augment the observations we made using the quantitative log analysis. More specifically we would like to:
\begin{enumerate}
\item	Quantify how common Deferral is and hence justify why we decided to study it in this work;
\item	Validate our assumption regarding the ties between the existence of Strong Actions and Deferral cases; That is, we are hoping to quantify the overlap between all emails that are deferred and all emails that are replied and identify whether taking strong actions on emails can be a reliable signal for deferral;
\item	Identify the reasons and motivations behind deferral;
\item	Identify the strategies people use to facilitate revisiting deferred emails and the ones they do not take in deferral scenarios
\end{enumerate}


